Efficient Wait-k Models for Simultaneous Machine Translation

Simultaneous machine translation consists in starting output generation before the entire input sequence is available. Wait-k decoders offer a simple but efficient approach for this problem. They first read k source tokens, after which they alternate between producing a target token and reading another source token. We investigate the behavior of wait-k decoding in low resource settings for spoken corpora using IWSLT datasets. We improve training of these models using unidirectional encoders, and training across multiple values of k. Experiments with Transformer and 2D-convolutional architectures show that our wait-k models generalize well across a wide range of latency levels. We also show that the 2D-convolution architecture is competitive with Transformers for simultaneous translation of spoken language.

==> details.tex <==
%Replicating the setup of~\cite{Elbayad18conll} for IWSLT14 De$\leftrightarrow$En, we train on 160K sentence pairs, develop on 7K held-out pairs and test on 6.7K pairs.
%The vocabulary consists of 8.8K types in German and 6.6K types in English that were obtained from a joint source and target byte pair encoding (BPE; \cite{Sennrich16acl}).
%We use the setup of \cite{Luong15iwslt} for IWSLT'15 Vi$\leftrightarrow$En.
%Apart from tokenizing the corpus, no other preprocessing step was done. The vocabulary sizes are 17K and 7.7K for English and Vietnamese respectively.
%For WMT15 De$\sto$En, we use setup of \cite{Ma19acl, Arivazhagan19acl} with a joint vocabulary of 32k BPE types.
%We train on 4.5M  pairs, develop on newstest2013 (3K pairs) and test on newstest15 (2.2K pairs).

%\mypar{Architectures}
%For the pervasive attention model, to reduce the memory footprint, we use residual skip connections~\cite{He16cvpr} rather than the dense connections~\cite{Huang17cvpr} used by \cite{Elbayad18conll}. 

%% MPA
%We consider a pervasive attention model (PA) that reads the source sequence bi-directionally via asymmetric convolution filters that are only masking the future targets.
%Note that this baseline is not directly applicable for low-latency decoding, due to the bi-directional source encoding.
%We use a uni-directional version of PA where the future source tokens are masked in the convolutions.

%% T
%For the Transformer model (TF), we use a \textit{small} architecture on IWSLT (De$\leftrightarrow$En, En$\leftrightarrow$Vi) with $d_\text{model}{=}256$ $N{=}6, d_{\mathrm{ff}}{=}1024, h{=}4,P_{\text{drop}}{=}0.3$.
%On WMT'15 De$\sto$En, we use a Transformer \textit{base} \cite{Vaswani17nips} with tied embeddings.
%Similar to pervasive attention (PA), we consider a model with a uni-directional encoder and a second model with a bi-directional encoder



